Cross-Chain State Machine Replication

This paper considers the classical state machine replication (SMR) problem in a distributed system model inspired by cross-chain exchanges. We propose a novel SMR protocol adapted for this model. Each state machine transition takes $O(n)$ message delays, where $n$ is the number of active participants, of which any number may be Byzantine. This protocol makes novel use of path signatures to keep replicas consistent. This protocol design cleanly separates application logic from fault-tolerance, providing a systematic way to replace complex ad-hoc cross-chain protocols with a more principled approach.

==> analysis.tex <==
\section{Analysis and Proof}


We have provided proof regarding initialization and bounded moves, here we give our proof regarding escrow related moves.


\begin{theorem}\label{theorem:onecompliant}
As long as there is a compliant party, then the blockchains either agree on the same escrow or they agree on no-response.
\end{theorem}

\begin{proof}
If there exists a compliant party, then the proposals on each blockchain are the same. If they agree on one escrow on one blockchain, the other blockchain must also decide on this escrow. If there is no agreement on one blockchain, it is the same on the other blockchain.
\end{proof}

\begin{theorem}
If the mover is compliant and all provers are compliant, then they agree on the same escrow.
\end{theorem}

\begin{proof}
By Theorem \ref{theorem:onecompliant}, we know all blockchains will either agree on the same escrow or a non-response. Since the mover is compliant, it will only propose one escrow, thus there is no challenge that happens. They will agree on the same escrow.
\end{proof}

\begin{theorem}
If the blockchain outputs a inconsistent move, the compliant competitor can leave the game with their assets.
\end{theorem}
\begin{proof}
By Theorem \ref{theorem:onecompliant}, we know the proposals on each blockchain are the same. If the blockchain outputs an escrow which is invalid, the compliant competitor has not proposed this escrow, thus the competitor can leave the game. The assets they have escrowed will be refunded. If the blockchain outputs non-response, the competitor cannot leave the game, however, it does not impact the competitor.
\end{proof}

\begin{theorem}\label{theorem:rejected}
If a mover is compliant, its move is either updated to the game on all blockchains or it is rejected which results in non-response.
\end{theorem}

\begin{proof}
If all provers are compliant, its move will be updated to the game since all provers proposed the same escrow. If not all provers are compliant, then some provers do not propose the escrow for the mover, then the mover's escrow will be refunded and the game will updated to non-response. In that case, a compliant mover's move is not correctly updated to the game. This is the compromise we make to guarantee consistence.
\end{proof}

Due Theorem \ref{theorem:rejected}, the game designer should carefully analyze the incentives for provers to be compliant and ensure the probability that all provers are compliant is very high. 





==> future.tex <==
distinguish broken state vs non response
discuss about parallel;
comparison vs other papers(cross-chain txn protocols, e.g. swap,cross-chain deals, lightning, auctions,token bridges)

==> optimization.tex <==
\section{Optimization: Parallel Execution}

The protocol proposed above all has a limit: to update a step, it requires at least N$\Delta$, due to the challenge phase required for any party to contest with a conflicting move. If there is a conflict, the move will be reduced to a non-response, and then players continue with the game based on this update. 

In some games, if there is no-response, the game also stops. In other words, if one party goes offline, the game should also stop since it is meaningless to continue. In that case, all parties just get their assets refunded(or there is another agreed upon payoff in that case). 
We can optimize our game by tentatively accept the current proposed step on that blockchain and make progress. When terminal state is reached, if there is still some step waiting to be finalized (i.e. in the challenge phase), it just wait until its challenge phase ends. If no successful challenge happens, the game is ended with the terminal state. If there is some successful challenge, then the game ends with the predefined payoff for that case.

By our optimization, suppose the game consists of $r$ rounds. Instead of taking $O(rN) \Delta$ rounds to compete the game, now we only need $O(r+N)\Delta$ to finish a game. 


==> premiums.tex <==
\section{Adding premiums to compensate honest players}

In case one party is not conforming and there are some victims identified, we can catch the nonconforming behavior and  let it pay a premium to compensate the victim.

For example, being non-responsive is a common deviating. The non-response behavior can be captured by the underlying blockchain which does not receive an available move in its buffer or receives more than one available move. In any case, we can let the party deposit a premium for being non-responsive. The consequence of a non-responsive move will be designed by the game designer.

Another nonconforming behavior is not approving an honest propose. This can also be captured by the underlying blockchain. If an available move is stored in the blockchain's buffer and a corresponding propose from a party $j$ is missing, then this party should pay a premium for not approving the behavior.

A third nonconforming behavior is leaving dishonestly. This is the same as the not approving an honest propose, which can be captured by the blockchain.

To sum up, a non-conforming behavior can be captured by the underlying blockchain which compares the proposals and the buffer. If they are not consistent or it is a no-response, the premium deposited should be distributed to victims.

==> protocols.tex <==
\section{Proposed State Machine Replication Protocols}
\subsection{Initial State}
To replicate the state among different blockchains, they should first agree upon an initial state. \textbf{The game cannot start if an initial state is not agreed upon all parties.} In the context of blockchains, since the game can be viewed as allocation of assets depending on states, usually the initial state consists of escrowing assets to be allocated later. During the game, new escrow may be allowed (e.g. an auction) or may not be allowed, denoted as bounded/unbounded budget game, respectively.  Depending on the number of initial states available to start the game and whether new escrow is allowed, the game from simple to complex can be categorized as: \begin{itemize}
    \item Univalent initial state, bounded budget game.
    \item Multivalent initial state, bounded budget game.
    \item Univalent initial state, unbounded budget game.
    \item Multivalent initial state, unbounded budget game.
\end{itemize}

 Univalent initial state means only predefined action(No response is always available, thus we do not count it in) is allowed for each party, i.e. escrow a predefined amount of assets. In that case, we can use a two-phase commit protocol to achieve an agreement between them. Multivalent initial state means parties can escrow different (amount of) assets and finally we want to reach an agreement between all parties which initial state they agree on to start with.


\paragraph{Univalent State Initialization}
Here we provide an initialization protocol to initialize a univalent initial state, shown in Alg ~\ref{alg:initialization1}.
\begin{algorithm}[htp!]
\caption{Univalent State Initialization}\label{alg:initialization1}
\begin{algorithmic}[1]
\Ensure A predefined state denoting each player's escrowed assets $s_0=(f_1^d,\cdots,f_i^d,\cdots f_n^d)$  where $f_j^{d}$ is the predefined funds for player $i$ or \textit{NoAgreement}

\Statex \textbf{Fund and Observe}


\Statex Within $\Delta$

\State Each player $i$ sends its escrow transaction $e(i,f^{d}_i)$ to the corresponding blockchain;

\State  Valid escrows $e(i,f^{d}_i)$ are included on the blockchains by miners and confirmed;

\State All parties observe each party's confirmed escrow
$e(i,f^{d}_i)$

\Statex \textbf{Commit}

\Statex Within $2\Delta$

\State Each honest player $i$ vote \textit{yes} to \textbf{all} blockchains if for $i\in[N]$, $e(i,f^{d}_i)$ is included on the corresponding blockchain.  Otherwise, do not do anything
\Statex \textbf{Relay}
\Statex Within $(N+1)\Delta$
\State Each player $i$ relays other's vote from one blockchain to all other blockchains if any vote is not shown on all blockchains, by signing on the vote of corresponding party.The timeout for a relaying vote(transaction) to be valid depends on number of signers in the signature. In short, we use path signatures to atomically commit.

\Statex \textbf{Decide}

\Statex After $(N+1) \Delta$

\Statex Decide the initial state on each blockchain:

\If{$ \forall j\in [1,N]$, the player $i$ votes yes
}

\State set the initial state as the univalent predefined state
$s_0=(f_1^d,\cdots,f_i^d,\cdots f_n^d)$


\Else
\If {$e(j,f_j)\neq 0$} in the smart contract
\State Refund the assets $f_j$

\Return {NoAgreement}
\EndIf
\EndIf

\Return {initial state $s_0$}

\end{algorithmic}
\end{algorithm}

Here, we use path signatures to atomically send one's vote to all blockchains. A path signature $\sigma_{v||p} =sig(\sigma_p,sk_v)$. That means, a party $v$ signs on a path signature associated with path $p(v\not p)$ with its own secret key $sk_v$. The timeout for a path signature depends on the number of parties in its path.


\begin{theorem}
As long as there exists a conforming party, then either all blockchains agree on $s_0=(f_1^d,\cdots,f_i^d,\cdots f_n^d)$ or all blockchains outputs no agreement.
\end{theorem}
\begin{corollary}
For any conforming party $i$,  either all blockchains agree on $s_0=(f_1^d,\cdots,f_i^d,\cdots f_n^d)$ or all blockchains outputs no agreement.
\end{corollary}



\begin{theorem}
If all parties are conforming, then the blockchains  agree on $s_0=(f_1^d,\cdots,f_i^d,\cdots f_n^d)$.
\end{theorem}


\paragraph{Multivalent Initial State Initialization}
For some games, players can choose to escrow different amount assets. For example, Alice can either escrow 10 tokens or 20 tokens depending on her decision. Then, the predefined initial state can have two values. All players have to decide on which initial state they start with. Here we show an initialization protocol if the initial state is multivalent, see Alg~\ref{alg:initialization2}.

\begin{algorithm}[htp!]
\caption{Multivalent Initial State Initialization}\label{alg:initialization2}
\begin{algorithmic}[1]

\Ensure An agreed upon state denoting each player's escrowed assets $s_0=(f^v_1,\cdots,f^v_i,\cdots f^v_n)$ where $f^v_i$ denotes player $i$'s escrow included on the blockchain or \textbf{NoAgreement}

\Statex \textbf{Funding$\&$Observe}


\Statex Within $\Delta$

\State Each player $i$ sends its escrow transaction $e(i,f_i)$ to the corresponding blockchain;

\State  Valid escrows $F^v=\{f^v_i\}_{i\in[1,N]} \subset F $ are included on the blockchains by miners and confirmed;

\State All parties observe each party's confirmed escrow
$F^v=\{f^v_i\}_{i\in[1,N]} \subset F $,

\Statex \textbf{Mover Propose}

\Statex Within $2\Delta$

\State Each player $i$ propose its action by sending a translated transaction of their escrow $T(e(j,F_j))$,i.e. the arguments they use to identify the move, signed by themselves $\sigma_j=sig(T(e(j,F_j)))$. They broadcast their proposal to all blockchains. 

\State Each party's proposal is included on blockchains in the proposal buffer which contains all proposals;

\Statex \textbf{Observer Propose}
\Statex Within $3\Delta$
\State Each observer $j$ proposes their opinion on each mover $i$'s move by signing on $\sigma_i$ corresponding to the escrow $e(i,F^i)$ included the blockchain, using their proposal secret keys $sk_j'$, thus sends $\sigma_{j||i}'=sig(\sigma_i,sk_j')$ to all blockchains. If there is no escrow for mover $i$, do not do anything.


\Statex \textbf{Challenge}
\Statex Within $(N+1) \Delta$
\State Each player $i$ relays other's proposal from one blockchain to all other blockchains if a proposal is in one blockchain's proposal buffer but is absent on another blockchain, by the path signature scheme. Those relayed proposals also reside in the proposal buffer.

\Statex \textbf{Decide}

\Statex After $(N+1) \Delta$

\Statex Decide the initialization on each blockchain:

\If{$ \forall j\in [1,N]$,  $ \forall i\in [1,N]$, there is only one distinguish signed $\sigma_{j||i}'$
}

\State set player $j$'s fund as $s_{0,j}=f_j$

\Else
\If {$e(j,f_j)\neq 0$ in the smart contract}
\State Refund the assets $f_j$

\Return {NoAgreement}
\EndIf
\EndIf

\Return {$s_0$}

\end{algorithmic}
\end{algorithm}

\begin{assumption}\label{assumption:initilization}
At least one player is conforming in the initialization phase.
\end{assumption}

\begin{theorem}\label{theorem:sameproposals}

By Assumption \label{assumption:initilization}, after $(N+1)\Delta$, all proposals shown on each blockchain are the same.
\end{theorem}
\begin{proof}
Suppose not. If there is one proposal $\sigma_{p}$ on one blockchain $C$ that does not show up on another blockchain $C'$, then the compliant party should not have signed $\sigma_{p}$. Then this compliant party can sign it and send it to $C'$ within one more $\Delta$ compared to the timeout of $p$.
\end{proof} 

\begin{theorem}\label{theorem:consensus}
By Assumption \label{assumption:initilization}, after initialization, all parties either agree on the same initial state across on all blockchains, or they abort the game due to \textbf{NoAgreement}.
\end{theorem}

\begin{proof} For any blockchain $C$, it outputs $s_0^{C}$ as the initial fund for all parties only if there is only one propose from all parties. That means, all parties only propose the same state for any player $j$. Otherwise, it output \textbf{NoAgreement}. 
\end{proof} 


\subsection{Moves}

After an initial state are agreed upon all parties, the parties can make moves to play the game. Recall that there are two kinds of games: bounded budget game and unbounded budget game. In bounded budget game, a move from available actions space is always valid to all blockchains, thus it does not need more verification. In unbounded budget name, a move from available actions space may not be valid to all blockchains, e.g. an escrow that exceed one's account balance. We call the later kind of moves as unbounded moves, and the former kind as bounded moves. We show how to replicate a move based on the type of the move.

\paragraph{Bounded Moves Replication}

Not surprisingly, the protocol to replicate their moves across different blockchains is similar to the initialization protocol.

\begin{algorithm}[htp!]
\caption{Move}\label{alg:moves}
\begin{algorithmic}[1]
%\Require A player $i\in N$ makes its move $mv$in its round or NoResponse

\Ensure An agreed upon state denoting this player's move or NoResponse

\Statex \textbf{Mover Propose}


\Statex Within $\Delta$

\State Player $i$ sends its proposed move $mv_i$(signed by player $i$, $\sigma_i=sig(mv_i,sk_i))$) to the all blockchains;

\State The proposal is included in the proposal buffer which contains all proposals;

\State All parties observe $mv_i$.


\Statex \textbf{Challenge}
\Statex Within $N \Delta$
\State Each player $j$ relays other's proposal from one blockchain to all other blockchains if a proposal is in one blockchain's proposal buffer but is absent on another blockchain, by the path signature scheme. Those relayed proposals also reside in proposal buffer.

\Statex \textbf{Decide}

\Statex After $N \Delta$

\Statex Decide the move on each blockchain:

\If{there is only one distinguish signed $mv_{i}$ shown up(not necessarily from all players)
}

\State set player $i$'s move to $mv_i$

\Else

\Return {NoResponse}
\EndIf

\Return {$mv_i$}

\end{algorithmic}
\end{algorithm}


\begin{assumption}\label{assumption:move}
At least one player is compliant for the move.
\end{assumption}
\begin{theorem}
By Assumption \ref{assumption:move}, after $N\Delta$, all proposals shown on each blockchain are the same.
\end{theorem}
Proof: the same as Theorem \ref{theorem:sameproposals}.
 
\begin{theorem}
By our Move algorithm, if conforming player $i$ makes one and only move $mv_i$, then all blockchains agree on that move. Otherwise, this step is marked as \textbf{NoResponse}.
\end{theorem}

\begin{proof}
For any blockchain $C$,  if it only sees one proposed $mv_i$, it outputs $mv_i$. If it sees another $mv_i'$, it will output NoResponse. If it does not see any $mv_i$, it also outputs NoResponse. 
\end{proof} 


\paragraph{Unbounded Moves Replication}

The unbounded moves replication poses new challenges. To avoid distraction,  we will use a new section to describe the challenge and our proposed solution, see Section \ref{escrow_in_game}.
\paragraph{State Transition by Timeout.} The state transition by timeout(denoted as non-response) is not automatically captured by smart contracts since smart contract cannot actively observe the clock on the blockchain and make the transition when time is out. The state transition by timeout must be triggered by a player who sends a transaction to proceed with the game or terminate the game. Only by this new transaction, the smart contract knows the clock of the outside world and then make "lazy" transitions. However, this "lazy" transition does not influence the correctness of our protocol. 


\subsection{Allocation on Terminal States}

When the game reached a terminal state, an allocation of assets is triggered. The allocation of assets depend on the moves from initial state to this terminal state. We assign an allocation function for each terminal state $s_t$ as $alloc(s_t)$. Then we set ownership of escrowed assets by $alloc(s_t)$. After the allocation function returns, players can send redeem transaction to redeem assets allocated to them. The redeem transaction can be any transaction signed by this party to show that they want to withdraw assets from the smart contract. We have this redeem transaction due to the fact that the smart contract cannot actively transfer assets to a party. The assets escrowed in the smart contract must be transferred to a party by some party actively calling a function.

Alg~\ref{alg:allocation} shows the Allocation algorithm.
\begin{algorithm}[htp!]
\caption{Allocation}\label{alg:allocation}
\begin{algorithmic}[1]
\Require A terminal state $s_t$, $owner[]$ denoting the owner of assets

\Ensure Ownership of assets in each contract

\For {$asset_i\in EscrowedAssets$}

\State owner[$asset\_i$] = $alloc(s_t,asset\_i)$

\EndFor

\Return {$owner[]$}

\end{algorithmic}
\end{algorithm}
One can redeem the assets by Alg~\ref{alg:redeem}.

\begin{algorithm}[htp!]
\caption{Redeem}\label{alg:redeem}
\begin{algorithmic}[1]
\Require A redeem transaction by player $i$ to redeem $asset_i$

\Ensure success or failure


\If {owner[$asset\_i$] = $i$}
\State Transfer $asset_i$ to $i$

\Return {Success}
\Else

\Return {Failure}
\EndIf

\end{algorithmic}
\end{algorithm}

\begin{comment}
\subsection{Replacing Move/Escrow By Secrets}

Suppose the moves are discrete and each move $j$ by a player $i$ can be represented by a secret $s_{i,j}$. Then in both initialization and move algorithms, we can replace the escrow and move transactions in the propose, challenge, and decide phase with hashlocks. If one party successfully escrowed or made a move on its own blockchain, then in the propose phase and later, it just release its secret as its proposal. That is, we match each action, including the steps taken during initialization to a hashlock. For each action, the corresponding player generates the hashlock and releases the hash and holds the secret(preimage).
\end{comment}


\subsection{Unbounded Budget Game}\label{escrow_in_game}

We have provided protocols for players to play a game if they escrow assets in the initialization phase and then only takes move in the game. Those moves are valid inherently bounded by the budget provided in the initial state. The protocols given above work for a wide range of cases. However, if during the game, players can escrow more assets, for example, in auctions, the above protocols does not work.

Moreover, we have the following challenge.
\subsubsection{Challenges}
The three properties in Def.\ref{properties} can be achieved if we assume there is a group of external nodes playing $\Pi$, among which, the majority of them are honest. Then we can use a majority rule to decide how to update the game view in each step.

However, in the case that the game is played among a group of players and no external nodes at hand, those players also play roles in $\Pi$ for state machine replication. The honest majority assumption does not hold anymore if sabotaging some properties gives particular parties advantage to improve their utility in playing the game.




\begin{theorem}
The three properties  in Def.\ref{properties} cannot hold if the number of Byzantine players in SMR protocol is arbitrary.
\end{theorem}

Proof: To ensure liveness, there is always one action(including no response) decided for each step. Assume a correct player sends an update $upd$ as their move. By fairness, the SMR protocol should decide $upd$, no matter how many players are Byzantine in playing $\Pi$, and send it to all blockchains. All blockchains should apply $upd$ on its own blockchain to update the game view. However, if a player sends an inapplicable but seemingly valid transaction $upd'$ as their move. By the same SMR protocol $\pi$, no matter how many players are Byzantine, the SMR protocol should also decide on $upd'$ since there is no additional information to $\Pi$ to tell that $upd'$ is inapplicable. Then consistency will be violated.



\paragraph{Reconcile Among Three Properties}

Since any SMR player can be Byzantine, those three properties cannot hold at the same time when some players become Byzantine. 

Can we guarantee two properties in Byzantine case? The answer is yes. We can guarantee consistency and liveness by outputting Non-response as a decision whenever the SMR players cannot reach an agreement on an update. In that case, we sacrifice fairness.

We can also guarantee liveness and fairness by outputting the proposed active move if SMR players cannot reach an agreement. In that case, we sacrifice consistency.

From the game theoretic perspective, what do two properties that we sacrifice mean?

If fairness is not provided, that means a player's move will be discarded and the game update would be a no-response for this step. Possibly the payoff is the least acceptable one. If a party is okay with the payoff caused by being discarded, the party can still play the game, only to keep in mind to check the payoff in the NP path in the game tree.


If consistency is not provided,  the game view on different chains diverge. Some players will be victims of this divergence since the game view on some chains is against them. In that case, we can provide an option to leave the game with a satisfying payoff. That means, we need to add transitions for players to leave the game and set payoff for those nodes.

Which property is preferred while the other property has to be sacrificed? For an agnostic move by a party in the game, different players prefer different properties. For example, the party(denoted as Prover) who makes the move favors fairness, and all other parties(denoted as Validators) favors consistency. It "seems" reasonable if we sacrifice Prover for the team due to utilitarianism. However, the consequence would be the Prover can never make a move according to his will due to some adversarial and competitors in the game. On the other hand, if we sacrifice the validators' consistency requirement and guarantee the prover's fairness, then the prover can always submit an inapplicable transaction, write it to the game, and break the consistency property. Then, every other party has to leave the game. This is also not expected since, now, the prover has control of the game and always maximize their own utility and make others leave.

Can we do better, i.e. try to accomplish fairness as best as possible and also try to guarantee consistency as best as possible?

Let us look closely at the problem. If fairness is provided, a party is always incentivized to cheat(by proposing an inapplicable transaction) if cheating maximizes their payoff. If consistency is provided, an adversarial party can always void an opponent's move if doing so maximizes their utility. The origin of the problem is that, while fairness backs one party up, it is hated by an opponent. The same situation works for consistency, too.

If in the game, there is one/more parties who love fairness and consistency both, we can break the tie. For example, in an auction where Alice is an auctioneer and Bob and Carol bid, Alice loves to see both of their bids and do not want any of their bids to be inapplicable(denoted as mutual party). Driven by that, we can let Alice decides the update. If Alice is honest, then fairness and consistency both are kept. If Alice is dishonest, fairness or consistency will be tampered, however bob and carol both accepts the payoff that Alice is dishonest. Since Alice has an incentive to be honest, we can assume with high probability, the game have the above three properties, and no one need to leave.

\begin{theorem}
If mutual parties exist, and a correct player makes an applicable move, then 
\begin{itemize}
    \item If all of prover's team is honest(with high probability), fairness is realized.
    \item consistency is also provided cause an applicable move is issued.
    \item If any of the prover's team is dishonest (with low probability), fairness is broken.
    
    \item In case that fairness is broken, the prover ends up a "least" acceptable payoff.

\end{itemize}

\end{theorem}

\begin{theorem}
If mutual parties exist, and an adversarial player makes an inapplicable move, then 
\begin{itemize}
    \item If \emph{any} of prover's team is honest(with high probability), consistency is guaranteed.
    \item If all of the prover's team are dishonest (with low probability), consistency is broken.
    
    \item In case that consistency is broken, the leavers ends up a "least" acceptable payoff.

\end{itemize}

\end{theorem}

What if there is no mutual party?

 For each agnostic update, each player can choose whether they favor fairness or consistency. If they favor fairness, they will be sided with the prover(with prover's invitation to side with them) and if an agreement is reached among them, the prover's transaction will be written to the game, and the other will be on the antagnistic team who may leave if they do not agree with prover's team. If there are only two opponent teams, the following case would happen.
 
 
 \begin{theorem}\label{theorem:compromise}
 
 For an update, if players either only care fairness to maximize their utility or anti fairness to maximize their utility, i.e. there is no mutual party, then one side have to compromise. 
 \end{theorem}
 
 Proof: if agreeing an agnostic update always benefits one side and hurts the other side, there is no mutual agreement for both of them. Then one side need to compromise.
 
Based on the result we get, we should have a new version of the game which extends the original game with new state transitions. For any escrow related move,  there is a designated voter committee to vote on the result of the move. Players outside this committee have a choice to leave the game with their assets. Thus, for any escrow related move, it may have the following transition: 1)no response, meaning the voter committee agree on no valid escrow happened 2) approved, and no other party leaves the game, or some parties leave the game.

\section{Extended Game}
Because of Theorem~\ref{theorem:compromise}, we have to add new transitions in the game. If a move is agnostic, we need to add transitions for competing players to leave the game. Also, we also need to update the payoff of player $i$ when their agnostic move is rejected and then they become a Byzantine player from the view of the game.
To sum up, when a state update is agnostic, we have two kinds of transitions:
\begin{itemize}
    \item Competing players can leave the game if the agnostic move is agreed upon by the prover's team. They should end up with an acceptable payoff.
    
    \item The prover's move is not agreed upon their team thus the move is a non-response. They should end up with an acceptable payoff.
\end{itemize}

We now take a second look what we want to accomplish in the new game.

When it is player $i$'s turn to make a move which is agnostic, to make a state update whether player $i$ makes a move, the SMR players are divided into two teams 1) Prover's team who has the right to propose the move, and once they agree upon an update, the state of the game is updated by their agreement.2) Competitor's team who has the right to leave the game if they see the game view is not consistent.

The game designer should design the game taking account in the new transitions.

The protocol to update game regarding an escrow related move is provided as in Alg. ~\ref{alg:escrow}. 

First, the game designer divides the players to prover's team and competitor's team.


\begin{algorithm}[htp]
\caption{Escrow As Move}\label{alg:escrow}
\begin{algorithmic}[1]

\Ensure A state update denoting player $i$ escrows $f^{u}_i$ with some competitor aborting the game or no one leaves the game OR a no-response denoting player $i$'s move is invalid or does not make a move at all. 

\Statex \textbf{Funding$\&$Observe}


\Statex Within $\Delta$

\State Each player $i$ sends its escrow transaction $e(i,f_i)$ to the corresponding blockchain;

\State  Valid escrows $F^v=\{f^v_i\}_{i\in[1,N]} \subset F $ are included on the blockchains by miners and confirmed;

\State All parties observe each party's confirmed escrow
$F^v=\{f^v_i\}_{i\in[1,N]} \subset F $,

\Statex \textbf{Mover Propose}

\Statex Within $2\Delta$

\State Each player $i$ propose its action by sending a translated transaction of their escrow $T(e(j,F_j))$,i.e. the arguments they use to identify the move, signed by themselves $\sigma_j=sig(T(e(j,F_j)))$. They broadcast their proposal to all blockchains. 

\State Each party's proposal is included on blockchains in the proposal buffer which contains all proposals;

\Statex \textbf{Observer Propose}
\Statex Within $3\Delta$
\State Each player $j$ proposes their opinion on each mover $i$'s move by signing on $\sigma_i$ corresponding to the escrow $e(i,F^i)$ included the blockchain, using their proposal secret keys $sk_j'$, thus sends $\sigma_{j||i}'=sig(\sigma_i,sk_j')$ to all blockchains. If there is no escrow for mover $i$, do not do anything.


\Statex \textbf{Challenge}
\Statex Within $(N+1) \Delta$
\State Any player $i$ relays other's proposal from one blockchain to all other blockchains if a proposal is in one blockchain's proposal buffer but is absent on another blockchain, by the path signature scheme. Those relayed proposals also reside in the proposal buffer.

\Statex \textbf{Decide}

\Statex After $(N+1) \Delta$

\Statex Decide the initialization on each blockchain:

\If{$ \forall j\in [1,N]$, there is \textbf{at most} one distinguish signed $\sigma_{j||i}'$
$\&\&$ $ \forall j\in provers$ , there is only one distinguish signed $\sigma_{j||i}'$} 

\State Set player $i$'s fund as $s_{m,i}=f_i$

\If{$s_{0,i}=f_i$ is not proposed by a competitor player $j$}

\State Refund the assets $f_j$
\State remove player $j$ in the game
\EndIf

\Return {${s_{m,i}}\&\&$ non-leaving parties}
\Else
\If {$e(i,f_i)\neq 0$ in the smart contract}
\State Refund the assets $f_i$

\Return {NoResponse}
\EndIf
\EndIf


\end{algorithmic}
\end{algorithm}


==> reconcile.tex <==


 

\begin{comment}

\section{High level abstraction}

Their are four roles in this game and state machine replication protocol:

1) game players; making moves or being byzantine to maximize their utility

2)nodes for SMR protocol

3) message system which send messages to all blockchains

4) blockchains, keep record of the update and apply those updates



From the example we see from Fig. ~\ref{fig:two_party_automaton}, we can see some moves are on one replica and some moves are on another, and some moves are on both replicas. Our goal is to replicate each replica's move to all other replicas so that each replica has the same view of the global state. How to do that?
Let us first look at the challenges in designing an SMR protocol. 
\begin{enumerate}
    \item Every move need to be atomically broadcast to all replicas. To do that, we can utilize the path signatures, and give 1 unit of $\delta$ for each appended signature. Compliant parties will forward any move that they see from one blockchain to all other blockchains. Thus, any move appear on one blockchain will eventually appear on all blockchains.
    \item If a state can accept multiple different inputs and transit to different new states, it is possible that two different blockchains receive different moves and then the views of two blockchains diverge. This problem can be fixed by requiring compliant players to broadcast any move they see to all blockchains, so that if there are two different moves at one position, the party that makes contradicting moves will be proven Byzantine and be punished. The victims will be compensated.
    \item The validity of some moves are not verifiable because of private information on each blockchain. For example, if Alice proposes that her move is escrow $x$ on apple blockchain to banana blockchain, which means that banana blockchain will write the escrow transaction to mirror what it thinks happened on banana blockchain. While on apple blockchain where Alice's escrow should happen, the escrow may not happen because of NotSufficientAmount. Thus, we should not only guarantee that the different replica has the same view of transactions appear on those blockchains, we should also take account of whether those transactions will be accepted by its local chain. If a transaction is rejected by its local chain, the common view constructed by transactions does not make sense anymore. However, if a transaction is rejected locally, we cannot prove it is rejected to other external blockchains to void this transaction. Here are two possible solutions:
    \begin{enumerate}
        \item Solution 1: Any valid move on its local blockchain is accepted. If a party's move is "silent" (by default), and it broadcasts a different(locally-invalid) move to other blockchains, other blockchains accept it as if it is true. Any compliant party who detect this divergence of views leave the game with its asset and a compensation due to this divergence for its trouble(we will show how to do that later).
        \item Solution 2: A move regarding private information on a local chain is decided by the votes of  parties. It is considered as valid as long as some designated parties have voted to confirm its validity. A compliant party who is not in the voting committee and sees a divergence can leave as the first case, and the remaining compliant parties can continue with the game. The drawback of this setting is that one compliant party may not be able to make a move at their will because the lack of confirmations from voting parties.
        
    \end{enumerate}
\end{enumerate}






\section{Decentralization-aware Game Tree(DAGT)}

The assumption that each blockchain can read other's blockchains' transactions do not hold.  So we should first translate the game trees to  decentralization-aware game trees. Typically, we can let parties broadcast transactions. Then, the thing is, because of private states in single blockchains, the other blockchain cannot verify the validity of an external transaction. An external transaction can be two types: a private value related transaction, e.g. an asset escrow where we do not know the budget from the account, and non private value related transaction. For the later type of transactions, every single blockchain can verify its validity and agree upon the next state. For the former type of transactions, each blockchain has its own opinion: on the blockchain that holds the private value, it knows its validity; on other blockchains, they do not know if the transaction is valid or not. There are two ways to resolve the dispute: 
\begin{enumerate}
    \item The external blockchains accepts it anyway, and the unhappy parties leave the game with their assets to avoid unhappy consequences by the dispute.  We call it accept-otherwise-leave option.
    
    \item  The external blockchain censors the transactions and only accepts it after censorship. For transactions that reside on the internal blockchain, if it does not pass censorship, those transactions will be voided. We call it censor-otherwise-void option.
\end{enumerate}





\section{From Decentralization-aware Game Trees to Cross-Chain protocols}
\section{Possible and Impossible Game Trees}
Suppose now we have 

\label{sec:headings}

\section{Problem with defining game trees}

Chess: tree too large;( may not be a problem, the rules are sufficient)
Auction: imperfect information about other's private value, utility function is also private. 

Solution: we do not care Nash equilibrium or their best strategies. We can replace the utility function as a payoff function which is public, only related to assets allocated in the game, regardless of their private values. And we can let each party only know its own payoff at terminal nodes.

Sequential steps: the last player can decide the final payoff (We need to introduce simultaneous games,i.e. rock-scissors-paper).


The pure games, e.x. prisoner's dilemma, it is assumed that there is a trusted coordinator. However, in the game played on computers, we need to make simultaneous step hidden at first and then release their steps.
\end{comment}

==> state_machine_replication.tex <==


\section{State Machine Replication}

We can treat the game as an application running a distributed database, where different cryptocurrencies reside on different replica(blockchain). Our goal is to make sure all replica has the same view of the state of the game globally. Before we dive into details, let us first look at why state machine replication across different blockchains are challenging.

\subsection{Challenge}

Suppose at any round of the game(we use round to denote it is a party's turn to make a move), a party chooses one available action and sends the corresponding transaction to all blockchains which will receive the transaction within a bounded time, the state machine replication can be achieved easily. However, since the parties are playing a game to maximize their utilities, parties are incentivised to cheat to make the game diverge if doing so gives them advantage. They can make the game on two blockchains inconsistent by only sending their transaction to one blockchain, or sending two different transactions to different blockchains, or sending invalid transactions(usually an escrow that exceeds its account balance) to a blockchain which seems to be valid from the view of the external blockchain. In that case, a consensus protocol must be run on top of their transactions to determine which transaction is made to update the game state. Due to the fact that we do not rely on trusted third parties to vote which update should be decided, the problem becomes more interesting when the update is decided by players in the game.

\subsection{Threat Models}
In this paper, the attack we consider is that a player tries to tamper the consistence of game on different blockchains. When it is a player $i$'s turn to make a move, it can launch:
\begin{itemize}
    \item Inconsistent transaction attack: meaning it sends two or more different actions to different blockchains
    \item Incomplete transaction attack: meaning it only sends its move to some blockchains, not all of them
    \item Invalid transaction attack: meaning it sends a locally invalid transaction to other blockchains and its local blockchain. Usually, a locally invalid transaction is an escrow whose validity depends on the local state(account balance) on the corresponding blockchain. There may be other locally invalid transactions whose validity is determined by local states.
\end{itemize}

Players also play roles in consensus to decide an update. A player can also launch attacks in the consensus procedure. The attacks will be obvious as we describe the consensus protocol.

\subsection{Communication Models}

To achieve the state machine replication, we first make some assumptions about our communication models.

\begin{assumption}\label{assumption:delay}

When a player sends a locally valid transaction to an associated blockchain,  within $\Delta$, the transaction will be included in a block and all other players can observe it.
\end{assumption}

\begin{corollary}

By Assumption \ref{assumption:delay}, if a locally valid transaction is sent to a blockchain $A$, then within $2\Delta$, the transaction can be written to any other blockchain $B$ if there exists a party relay it to blockchain $B$.

\end{corollary}

\begin{assumption}
The clocks on different blockchains are synchronized (For simplicity, denoted as SyncClock). That means, there is no clock skew between different blockchains.\footnote{In practice, blockchains have small clock skew(at most a few minutes)among them. Since $\Delta$(order of hours) is way larger then the clock skew, the clock skew does not affect the correctness}
\end{assumption}
\subsection{State Machine Replication Requirements}
The State Machine Replication (SMR) protocol we design aims to achieve the following goals. Game view means the state update in the state machine.

\begin{definition}\label{properties}
An SMR protocol $\Pi$ deciding the update (deterministically decided by the current state and the inputs) of state machine should satisfy the following properties:
\begin{itemize}
    \item Consistency. Every blockchain agrees on the same move at step $i$.
    \item Liveness. The blockchains eventually agree upon an update.
    \item Fairness.  A move by a correct party is eventually written to the game view.
\end{itemize}
\end{definition} 

